Rivalry of Two Families of Algorithms for Memory-Restricted Streaming PCA

We study the problem of recovering the subspace spanned by the first $k$ principal components of $d$-dimensional data under the streaming setting, with a memory bound of $O(kd)$. Two families of algorithms are known for this problem. The first family is based on the framework of stochastic gradient descent. Nevertheless, the convergence rate of the family can be seriously affected by the learning rate of the descent steps and deserves more serious study. The second family is based on the power method over blocks of data, but setting the block size for its existing algorithms is not an easy task. In this paper, we analyze the convergence rate of a representative algorithm with decayed learning rate (Oja and Karhunen, 1985) in the first family for the general $k>1$ case. Moreover, we propose a novel algorithm for the second family that sets the block sizes automatically and dynamically with faster convergence rate. We then conduct empirical studies that fairly compare the two families on real-world data. The studies reveal the advantages and disadvantages of these two families.

==> preliminary.tex <==
\section{Preliminaries}
Without loss of generality, we make the following assumptions
\begin{itemize}
  \item The $\bx \in \mathbb{R}^d$ are i.i.d with mean zero and covariance $A$.
  \item There is a constant $b$ such that $\|\bx\|^2 \leq b$
  \item The eigenvalues $\lambda_1\geq\lambda_2\geq \cdots \geq\lambda_d$, and $\lambda_i>\lambda_{i+1}$.
\end{itemize}

Also, let $U$ denote the $d\times k$ matrix consisting of the $k$ singular vectors of $A$ as columns, and let $\ort{U}$ denote the $d\times (n-k)$ matrix consisting of the remaining $n-k$ singular vectors of $A$ as columns. Let $\alpha$ denote the $k$-th singular value of $A$ and let $\ort{\alpha}$ denote the $(k+1)$-th one.

For a vector $\bx$, we let $\|\bx\|$ denote its $\ell_2$-norm. For a matrix $M$, we will consider the following two different norms:
$$\|M\| = \max_{\bx} \frac{\|M\bx\|}{\|\bx\|} \mbox{  and  } \lambda_{\min}(M) = \min_{\bx} \frac{\|M\bx\|}{\|\bx\|}.$$

\subsection{Error Measure}
In~\cite{fastpca}, the adopted error measure for the rank-1 case is 
\[
  \Psi_t = 1-\frac{(U^TQ_t)^2}{\|Q_t\|^2}.
\]
Note that both $U$ and $Q_n$ are vectors in the rank-1 case.
The analogue error for the general rank-$k$ case can be defined as
\[
  \Psi_t = 1-\lminq{U^TQ_t}.
\]
If $k$ is $1$, then these two error measures are exactly the same.

On the other hand, in~\cite{MCJ13}, the error measure is defined as
\[
  \Psi_t = \|\ort{U}^TQ_t\|.
\]

\begin{lemma}Principal angle~\textnormal{\citep{m_comp}}\label{lem:sub_equ}
  $1-\lminq{U^TQ}=\|\ort{U}^TQ\|^2$
\end{lemma}

From Lemma~\ref{lem:sub_equ}, these two measures are exactly the same. In this paper, we will use them interchangeably.
Also, to simplify the notation, we define 
$$V_t = U^\top Q_t \mbox{ and }\ort{V}_t = \ort{U}^\top Q_t.$$

\subsection{Nested Sample Space}
Let $\mathcal{F}_n$ denote the sigma-field of all outcomes up to and including time $n$, that is,
$\mathcal{F}_n = \sigma(\mathbb{Q}_0, \mathbb{X}_0,\cdots,\mathbb{X}_n)$. Also, let $\Omega$ 
denote the sample space of all realizations $(Q_0, \bx_0, \bx_1, \cdots)$, and P the
probability distribution on these sequences. For any $\delta>0$, we define a nested sequence of spaces
$\Omega\supset\Omega_0'\supset\Omega_1'\cdots$ such that$\Omega_n'$ is $\mathcal{F}_{n-1}$ measurable,
has probability $\pr{\Omega_n'} \geq 1-\delta$.

